When Transparency Backfires: Corruption in Cooperative Multi-Agent Systems

Can transparency sustain cooperation in collaborative environments where agents may establish private influence channels to monitoring AI agents? We studied 4,320 repeated five-player bribery games in which members may direct transfers to leaders tasked with maintaining cooperation. GPT-5.6 Luna leaders imposed smaller fines on free riders who offered bribes, even when instructed to prioritize group earnings. In Claude Haiku 5.5 groups, members rarely offered bribes to leaders, yet leaders failed to calibrate punishments thereby eroding the gains from cooperation. Disclosing past contributions, offers to the leader, acceptance decisions, and fines had mixed effects on agent contributions. When a single adversary offered a minimal bribe to the leader while free riding, disclosure significantly reduced group earnings. Our findings suggest that institutional robustness depends on both enforcement integrity to keep private gains from distorting sanctions and enforcement calibration to ensure that sanctions sustain enough cooperation to justify their collective cost. Oversight mechanisms should be imposed with attention to the group dynamics they induce and the consequences of those dynamics for collective welfare.

==> subsections/6.power-and-potential.tex <==
\subsubsection{Enforcement Power and Economic Potential}
